Resonant Hamiltonian systems associated to the one-dimensional nonlinear Schr\"odinger equation with harmonic trapping

We study two resonant Hamiltonian systems on the phase space $L^2(\mathbb{R} \rightarrow \mathbb{C})$: the quintic one-dimensional continuous resonant equation, and a cubic resonant system that has appeared in the literature as a modified scattering limit for an NLS equation with cigar shaped trap. We prove that these systems approximate the dynamics of the quintic and cubic one-dimensional NLS with harmonic trapping in the small data regime on long times scales. We then pursue a thorough study of the dynamics of the resonant systems themselves. Our central finding is that these resonant equations fit into a larger class of Hamiltonian systems that have many striking dynamical features: non-trivial symmetries such as invariance under the Fourier transform and the flow of the linear Scr\"odinger equation with harmonic trapping, a robust wellposedness theory, including global wellposedness in $L^2$ and all higher $L^2$ Sobolev spaces, and an infinite family of orthogonal, explicit stationary wave solutions in the form of the Hermite functions.

==> cr/art-app-A.tex <==


Theorem \ref{thm:3:maxE} has two distinct parts,
 which we state here independently as Lemma \ref{thm:A:decomp} and Theorem \ref{thm:A:equality}.

\begin{lemma}[Decomposition Lemma]
	\label{thm:A:decomp}
	Let $A$ be an isometry.
	Denote $\tilde{f}_k(x) = f_k(-x)$.
	There exists integers $m$ and $l$, with $0 \leq m \leq l \leq n$, and two permutations $\sigma_1$ and $\sigma_2$ of the integers $\{1,\ldots,n\}$
	such that,
	\begin{align*}
		E_A(f_1,\ldots,f_{2n}) &= 
			\left( \prod_{k=1}^m \jap{f_{\sigma_1(k)}, f_{n+\sigma_2(k)} }	\right)
			\left( \prod_{k={m+1}}^l \jap{f_{\sigma_1(k)}, \tilde{f}_{n+\sigma_2(k)} } \right)	\\
			& \hspace{2.5cm} \times E_B(
				f_{\sigma_1(l+1)},\ldots
				f_{\sigma_1(n)},
				f_{n+\sigma_2(l+1)},\ldots
				f_{n+\sigma_2(n)}),
	\end{align*}
	where the matrix $B:\R^{n-l} \rightarrow \R^{n-l}$ has no permutation part; that is, for all $i$ and $j$, $Be_i \neq \pm e_j$.
\end{lemma}


\newcommand{\sok}[1]{e_{\sigma_1(#1)}}
\newcommand{\stk}[1]{e_{\sigma_2(#1)}}

\begin{proof}
	Call a pair of integers $(i,j)$ good if $Ae_i = e_j$ and bad if $Ae_i=-e_j$.
	Because $A$ is injective, for a given $j$ there is at most one $i$ such that $(i,j)$ is good or bad.
	Let $m$ be the number of good pairs, and $l-m$ the number of bad pairs.
	Order the good pairs in any way, and for $k=1,\ldots,m$, 
		let $\sigma_1(k)=i$ and $\sigma_2(k)=j$ where $(i,j)$ is the $k$th good pair in the ordering.
	In a similar fashion, order the bad pairs in any way, and for $k=l+1,\ldots,m$,
		let $\sigma_1(k)=i$ and $\sigma_2(k)=j$ where $(i,j)$ is the $(k-m)$th bad pair in the ordering.

	Now consider $i$ such that $i$ is not the first component in a good or bad pair. 
	%(One is tempted to call such an $i$ ugly.)
	There are $n-l$ such $i$.
	Order them in any way, and for $k=l+1,\ldots,n$ set $\sigma_1(k)=i$ where $i$ is the $(k-l)$th number in the ordering.
	Then consider $j$ such that $j$ is not the second component in a good or bad pair, and
		for $k=l+1,\ldots,n$ define $\sigma_2(k)=j$ in a similar fashion.

	It is clear that,
	\begin{align}
		A: 
		&\text{span}( \sok{1},\ldots,\sok{m} ) \cong \R^m \rightarrow
		\text{span}( \stk{1},\ldots,\stk{m} ) \cong \R^m	\label{eqn:A:Sp}	\\
		A: 
		&\text{span}( \sok{m+1},\ldots,\sok{l} ) \cong \R^{l-m} \rightarrow
		\text{span}( \stk{m+1},\ldots,\stk{l} ) \cong \R^{l-m}, \label{eqn:A:Sn}
	\end{align}
	and that $A=I$ and $A=-I$ on these subspaces respectively, with the implied identifications of bases.
	Because $A$ is an isometry, we then necessarily have,
	\begin{equation}
		A: 
		\text{span}( \sok{m+1},\ldots,\sok{n} ) \cong \R^{n-m} \rightarrow
		\text{span}( \stk{m+1},\ldots,\stk{n} )	\cong \R^{n-m}.
		\label{eqn:A:Sc}
	\end{equation}
	Let $B$ be the restriction of $A$ as a map between the subspaces in \eqref{eqn:A:Sc}.
	The condition that $Be_i \neq \pm e_j$ holds because otherwise $(i,j)$ would be a good or bad pair and $e_i$ and $e_j$ would not be in the subspaces given in \eqref{eqn:A:Sc}.
	
	The representation of $E_A$ arises because $A$ is the identity in \eqref{eqn:A:Sp} and the negative of the identity in \eqref{eqn:A:Sn}.
\end{proof}


In light of the representation of $E_A$, it is clear that we have the equality
	 $|E_A(f_1,\ldots,f_{2n})| = \prod_{k=1}^{2n} \|f_k\|_{L^2}$
if and only if the following three conditions hold.
\begin{enumerate}
	\item For all $k=1,\ldots,m$, 
		$|\jap{ f_{\sigma_1(k)}, f_{n+\sigma_2(k)} }| = \| f_{\sigma_1(k)} \|_{L^2} \| f_{n+\sigma_2(k)} \|_{L^2} $, which means 
		$f_{\sigma_1(k)} = C_k f_{n+\sigma_2(k)} $ for some constant $C_k$ by the usual \CS{} equality condition.
	\item For all $k=m+1,\ldots,l$, 
	    \[
            |\jap{ f_{\sigma_1(k)}, \tilde{f}_{n+\sigma_2(k)} }| 
            = \| f_{\sigma_1(k)} \|_{L^2} \|\tilde{ f}_{n+\sigma_2(k)} \|_{L^2} 
            = \| f_{\sigma_1(k)} \|_{L^2} \| f_{n+\sigma_2(k)} \|_{L^2},
            \] which means 
		$f_{\sigma_1(k)} = C_k \tilde{f}_{n+\sigma_2(k)} $ for some constant $C_k$, again by the usual \CS{} equality condition.
	\item	$ |E_B(
				f_{\sigma_1(l+1)},\ldots
				f_{\sigma_1(n)},
				f_{n+\sigma_2(l+1)},\ldots
				f_{n+\sigma_2(n)})| = \prod_{k=l+1}^n   \| f_{\sigma_1(k)} \|_{L^2} \| f_{n+\sigma_2(k)} \|_{L^2}$
\end{enumerate}
To finish the proof of Theorem \ref{thm:3:maxE}, we examine the equality case in item 3.
This equality is, of course, identical looking to the original equality condition \eqref{eqn:3:cseq}.
The difference is that $B$ has the structural condition $Be_i \neq \pm e_j$.


\begin{thm}
	\label{thm:A:equality}
	Suppose that $A$ is an isometry, and for all $i$ and $j$, $Ae_i \neq \pm e_j$.
	 Then, $$|E_A(f_1,\ldots,f_{2n})| = \prod_{k=1}^{2n} \|f_k\|_{L^2},$$
	 only if each of the functions is a Gaussian.
	Equality holds if each of the functions is the same Gaussian of the form $e^{-\alpha x^2}$ for some $\alpha>0$.
\end{thm}


The `if' part of the Theorem was proved before, in Theorem \ref{thm:3:maxH}.
The `only if' part follows from a close analysis of the  \CS{} equality condition,
\begin{equation}
	\prod_{k=1}^n f_k ((Ax)_k)=
	\prod_{k=1}^n f_{n+k}( x_k ),
	\label{eqn:A:CS}
\end{equation}	
which was given in \eqref{eqn:3:cseq}.
The proof is in three steps.
\begin{enumerate}
	\item First we show that if all the functions in \eqref{eqn:A:CS} are smooth and strictly positive, then
		they must be Gaussians.
	\item Next we show that if all the functions in \eqref{eqn:A:CS} are merely non-negative and in $L^2$,
		then they must be Gaussians.
		The idea here is extremely simple: the heat flow acting on each function simultaneously conserves the relationship \eqref{eqn:A:CS}.
		For future times, the heat flows are smooth and positive, and part one can be applied.
	\item Finally we show that if the functions in \eqref{eqn:A:CS} are complex valued and in $L^2$,
		then they must be Gaussians.
\end{enumerate}


\begin{lemma}[Step One]
	Suppose that functions $f_k$ satisfy \eqref{eqn:A:CS}, are all strictly positive and  smooth.
	Then they are all Gaussians. 
\end{lemma}

\begin{proof}
	Let $g_k(x) = \log f_k(x)$.
	Because $f_k$ is strictly positive and smooth, $g_k$ is well-defined and smooth.
	To show $f_k$ is a Gaussian we will show that $g_k$ is polynomial of degree at most two.

	Because $A$ is an isometry, it satisfies $A^{-1}=A^T$.
	Therefore, for all $m$, we have the matrix expansions,
	\begin{align}
		A e_m &= \sum_{k=1}^n a_{km} e_k \;\;\text{ and }\;\;
		A^{-1} e_m = \sum_{k=1}^n a_{mk} e_k,
		\label{eqn:A:Aaction}
	\end{align}
	for numbers $ \{ a_{km} \}_{k,m=1}^n$.
	By the assumptions in the theorem, we have $|a_{km}|<1$ for all $k$ and all $m$.
	Set $\epsilon=\max_{m,k} | a_{km} |<1$.
	Because $A$ is an isometry, we have,
	\begin{equation}
		1 = |Ae_m|^2 =
		\sum_{k=1}^n a_{km}^2 
		\;\;\text{ and }\;\;
		1 = |A^{-1}e_m|^2 =
		\sum_{k=1}^n a_{mk}^2 ,
		\label{eqn:A:Aisom}
	\end{equation}
	for all $m$.
		

	Taking the logarithm of both sides of the \CS{} equality condition \eqref{eqn:A:CS} (and switching the left and right sides) 
		gives the condition on the functions $g_k$,
	\begin{equation}
		\sum_{k=1}^n g_{n+k}(x_k) = 
		\sum_{k=1}^n g_k( (Ax)_k ). 
		\label{eqn:3:CSforg}
	\end{equation}
	Fix $m \in \{1,\ldots,n\}$ and set $x= t e_m$.
	For all $k\in \{1,\ldots,n\}$,
	we have $(Ax)_k=t(Ae_m)_k = ta_{mk}$ and $x_k = t \delta_{km}$.
	Therefore,
	\[
		g_{n+m}(t) + \sum_{\substack{k=1 \\ k\neq m}}^n g_{n+k}(0) = 
		\sum_{k=1}^n g_k( a_{km}t ).
	\]
	Differentiating this equation twice with respect to $t$ yields,
	\begin{equation}
		g_{n+m}''(t) =
		\sum_{k=1}^n a_{km}^2 g_k''( a_{km}t ) .
		\label{eqn:3:gsd0}
	\end{equation}
	We can evaluate this equation at $t=0$ to get
		$ g_{n+m}''(0)  = \sum_{k=1}^n a_{km}^2 g_k''( 0 ) $.
	Subtracting this from \eqref{eqn:3:gsd0} then gives,
	\begin{equation}
		g_{n+m}''(t) - g_{n+m}''(0) =  \sum_{k=1}^n a_{km}^2 \left[ g_k''( a_{km}t )-g_k''(0) \right].
		\label{eqn:3:gsd}
	\end{equation}
	For all indices $m$ and $k$ we have $a_{km}t \in [-\epsilon|t|,\epsilon|t|]$ and so the bound,
	\begin{equation}
		|g_{n+m}''(t) - g_{n+m}''(0)| \leq 
			\max_{s \in [-\epsilon|t|,\epsilon|t|]}
			\max_{k=1,\ldots,n} 
			|g_k''(s)-g_k''(0)|,
		\label{eqn:3:bound1}
	\end{equation}
	holds for all $m \in \{ 1,\ldots,n \}$.

	The \CS{} equality condition is similar when the roles of  $f_1,\ldots,f_n$ and $f_{n+1},\ldots,f_{2n}$ are switched.
	This may be seen by replacing $x$ by $Ax$ and finding,
	\begin{equation}
		\prod_{k=1}^n f_{n+k} ((A^{-1}x)_k)=
		\prod_{k=1}^n f_{k}( x_k ),
		\label{eqn:A:CS2}
	\end{equation}	
	By equations \eqref{eqn:A:Aaction} and \eqref{eqn:A:Aisom}, the same estimates for $A$ hold for  $A^{-1}$.
	Therefore, performing the same argument as before, we find,
	\begin{equation}
		|g_{m}''(t) - g_{m}''(0)| \leq \max_{s \in [-\epsilon|t|,\epsilon|t|]} \max_{k=1,\ldots,n} |g_{n+k}''(s)-g_{n+k}''(0)|
		\label{eqn:3:bound2}
	\end{equation}
	for all $m \in \{1,\ldots,n\}$.

	The two families of inequalities \eqref{eqn:3:bound1} and \eqref{eqn:3:bound2} may be combined into one inequality,
	\begin{equation}
		\max_{k=1,\ldots,2n} |g_{k}''(t) - g_{k}''(0)| \leq \max_{s \in [-\epsilon|t|,\epsilon|t|]} \max_{k=1,\ldots,2n} |g_{k}''(s)-g_{k}''(0)|
		\label{eqn:3:bound3}
	\end{equation}
	This holds for all $t$.
	Applying it recursively $N$ times yields
	\begin{equation*}
		\max_{k=1,\ldots,2n} |g_{k}''(t) - g_{k}''(0)| \leq \max_{s \in [-\epsilon^N|t|,\epsilon^N|t|]} \max_{k=1,\ldots,2n} |g_{k}''(s)-g_{k}''(0)|.
		%\label{eqn:3:bound3}
	\end{equation*}
	But now $\epsilon<1$, and so we have, because $g$ is smooth,
	\begin{align*}
		\max_{k=1,\ldots,2n}
		|g_{k}''(t) - g_{k}''(0)| 
		&\leq \lim_{N \rightarrow \infty} 
			 \max_{s \in [-\epsilon^N|t|,\epsilon^N|t|]} \max_{k=1,\ldots,2n} |g_{k}''(s)-g_{k}''(0)|	\\
		&= \max_{k=1,\ldots,2n} |g_{k}''(0)-g_{k}''(0)|	 = 0.
	\end{align*}
	Hence $g_k''(x)=g_k''(0)$ is a constant, $g_k(x)$ is a polynomial of degree at most two,
		and $f_k(x) = e^{g_k(x)}$ is a Gaussian.
\end{proof}

The proof of the previous lemma required smoothness and positivity assumptions on the $f_k$ functions.
We now use a heat flow argument to upgrade the result to non-smooth and non-negative $f_k$.

\begin{lemma}[Step two, part one]
	The \CS{} equality condition \eqref{eqn:A:CS} is conserved by the heat flow.
	More precisely, suppose that there is a $\gamma>0$ such that all of
		the functions in \eqref{eqn:A:CS} satisfy $f_k e^{-\gamma x^2} \in L^1$.
	Then there is a time $T$ such that the heat flow $e^{-t\Delta}f_k$ is defined for $t\in(0,T)$ and all $k$.
	For fixed $t\in(0,T)$ the functions $h_k(x) =  (e^{-t\Delta}f_k)(x)$ satisfy \eqref{eqn:A:CS}.
\end{lemma}


\begin{proof}
	Under the assumptions on $f_k$ we can write the solution of the heat equation $e^{-t\Delta}f_k$
	 using the fundemental solution as,
	\[
		(e^{-t\Delta}f_k)(x_k) = \frac{1}{\sqrt{ 4\pi t}} \int_\R e^{-|y_1|^2/4t} f(x_k-y_k) dy_k.
	\]
	The formula is well defined for $0<t<T$, with $T<1/\gamma$, because of the integrability assumptions on $f_k$.
	Using this formula $n$ times, we have,
	\begin{align*}
		\prod_{k=1}^n (e^{-t\Delta}f_k)( (Ax)_k ) 
			& = \frac{1}{ (4\pi t)^{n/2} } \int_{\R^n} e^{-|y|^2/4t}  \prod_{k=1}^n f_k((Ax)_k-y_k) dy \\
			& = \frac{1}{ (4\pi t)^{n/2} } \int_{\R^n} e^{-|y|^2/4t}  \prod_{k=1}^n f_k((A(x-A^{-1}y))_k) dy \\
			& = \frac{1}{ (4\pi t)^{n/2} } \int_{\R^n} e^{-|y|^2/4t}  \prod_{k=1}^n f_{n+k}((x-A^{-1}y)_k) dy,
	\end{align*}
	where in the last line we have used the \CS{} equality condition \eqref{eqn:A:CS}.
	We now perform the change of variables $z=A^{-1}y$. 
	Because $A$ is an isometry, the determinint of this change of variables is 1,
		and we also have $|y| = |Az| = |z|$ for every $y \in \R^n$.
	This gives,
	\begin{align*}
		\prod_{k=1}^n (e^{-t\Delta}f_k)( (Ax)_k ) 
			 = \frac{1}{ (4\pi t)^{n/2} } \int_{\R^n} e^{-|z|^2/4t}  \prod_{k=1}^n f_{n+k}(x_k - z_k) dy	
			= 
		\prod_{k=1}^n (e^{-t\Delta}f_{n+k})( x_k ).
	\end{align*}
	For fixed $t$ the maps $h_k(x) =  e^{-t\Delta} f(x)$ thus satisfy \eqref{eqn:A:CS}.
\end{proof}



\begin{corr}[Part two, step two]
	Suppose that non-negative functions $f_k \in L^2$ satisfy \eqref{eqn:A:CS}.
	Then all of the functions are Gaussians.
\end{corr}

\begin{proof}
	If $f_k\in L^2$, then $f_k e^{-\gamma x^2}\in L^1$ for all $\gamma>0$.
	By the previous lemma, the heat flow $e^{-t\Delta}f_k$ exists for all $k$ and $t \in (0,\infty)$,
	and the functions $h_k(x) = e^{-t\Delta}f_k(x)$ satisfy \eqref{eqn:A:CS}.
	The functions $h_k$ are smooth, and because the initial data is non-negative, the functions $h_k$ are also positive.
	By the first lemma, each of the $h_k$ functions are Gaussians.

	Fix $k$.
	By substituting the general form of a time dependent Gaussian into the heat equation we discover that
		if $e^{t\Delta}f_k$ is a Gaussian for all $t\in(0,T)$ then necessarily, for $t>0$,
	\[
		(e^{-t\Delta}f_k)(x) = \frac{d}{\sqrt{t+a}} e^{-b(x-c)^2/4(t+a)},
	\]
	for some $a\geq 0$ and $b,d>0$ and $c \in \R$. We calculate,
	\[
		\| e^{-t\Delta} f_k \|_{L^2}^2 = \frac{d^2}{t+a} \int_\R e^{-b(x-c)^2/2(t+a)} dx =
			\frac{d^2}{\sqrt{t+a}} \sqrt{ \frac{2\pi}{b} }.
	\]
	Then, because $\|e^{-t\Delta}f_k \|_{L^2} \leq \| f_k \|_{L^2}$, we must have $a>0$.
	This gives
	\[
		f_k(x) = \lim_{t \rightarrow 0} (e^{-t\Delta}f_k)(x) = \frac{1}{\sqrt{a}} e^{(bx^2 + cx)/4a)},
	\]
	so $f_k$ is a Gaussian.
\end{proof}

Having proved the result for non-negative $f_k$ we lastly prove it for general complex valued $f_k$.


\begin{lemma}[Step three]
	Suppose that functions $f_k \in L^2$ satisfy \eqref{eqn:A:CS}.
	Then all of the functions are Gaussians.
\end{lemma}


\begin{proof}
	We assume that the functions $f_k$ are smooth; the result for general functions follows from invoking the heat flow argument as in Step Two.

	Taking absolute values in the equality condition \eqref{eqn:A:CS},
		we see that the functions $|f_k|$ satisfy the condition as soon as the functions $f_k$ do.
	By the previous Lemmas, $|f_k|$ must be a Gaussian $G_k(x)$ for all $k$, and hence
	\begin{equation}
		f_k(x) = e^{ig_k(x)}G_k(x),
		\label{eqn:3:complexf}
	\end{equation}
	for some real valued function $g_k$. 
	Note that from this we necessarily have $f_k(x) \neq 0$.
	Because $f_k$ and $G_k$ are smooth, and
	$e^{ig_k(x)} = f_k(x) / G_k(x)$ 
	we can choose $g_k$ to be smooth.

	Plugging the expressions \eqref{eqn:3:complexf} for $f_k$ into \eqref{eqn:A:CS} we find
	\[
		\prod_{k=1}^n e^{ig_k( (Ax)_k )} G_k( (Ax)_k)
		=\prod_{k=1}^n e^{ig_{n+k}( x_k )} G_{n+k}( x_k).
	\]
	The $G_k$ terms cancel because we know the functions $G_k = |f_k|$ also satisfy \eqref{eqn:A:CS}.
We are left with $e^{i \sum_{k=1}^n g_k( (Ax)_k ) } = e^{i \sum_{k=1}^n g_k(x_k)}$, and hence
\[
	\sum_{k=1}^n g_k( (Ax)_k ) =  \sum_{k=1}^n g_{n+k}(x_{k}) + 2\pi n(x).
\]
where $n :\R^n \rightarrow \mathbb{Z}$. Because $g$ is smooth, $n$ is smooth and  hence a constant.
Plugging in $x=0$ gives $n(x) =0$, and then the equation for the functions $g_k$ is thus,
\[
	\sum_{k=1}^n g_k( (Ax)_k ) =  \sum_{k=1}^n g_{n+k}(x_k).
\]
This is precisely equation \eqref{eqn:3:CSforg}.
As before, $g_k$ must be a polynomial of degree at most two, and $f_k$ is a complex Gaussian.
\end{proof}


==> cr/art-chp-3.tex <==

In the introduction we presented
	two formulas
	\eqref{eqn:1:quinticHam} and \eqref{eqn:1:cubicHam} that
	represent the Hamiltonians $\Ham_6$ and $\Ham_4$ in terms of simpler functionals of the form $E_A$,
\begin{align}
	\Hqin(f) &= \frac{1}{2\sqrt{3} \pi^2} \int_0^{2\pi} E_{R(\theta)}(f,f,f,f,f,f) d\theta, \\
	\Hcub(f) &= \frac{1}{2\sqrt{2} \pi^2} \int_0^{2\pi} E_{S(\theta)}(G,f,f,G,f,f) d\theta.
	\label{eqn:3:hams}
\end{align}
Here, for an isometry $A: \R^n \rightarrow \R^n$, %which for us will always be an isometry, 
	the $2n$ multilinear functional $E_A$ is defined by,
\begin{equation}
	E_A(f_1,\ldots,f_{2n}) 
		= \int_{ \R^n } \prod_{k=1}^n f_k( (Ax)_k ) \of_{n+k}( x_k ) dx,
	\label{eqn:3:EA}
\end{equation}
where $x\in \R^n$, $x_k = \jap{ x, e_k }$ and $(Ax)_k = \jap{ Ax, e_k }$.
(In the introduction, and in formulas \eqref{eqn:3:hams}, $n$ is set to $3$, but the work in this section is for arbitrary $n$.)
As stated in the introduction, 
	it turns out that one can gain significant insight into the dynamics of the systems associated to the Hamiltonians $\Ham_6$ and $\Ham_4$
	by understanding properties of the functionals $E_A$.
This section, therefore, is a general study of this family of functionals.
We will examine the symmetries of $E_A$, its boundedness in $L^2$ and higher Sobolev spaces, and 
	its relationship to the Hermite functions. 
Our motivation throughout is to relate these findings back to the dynamics of the Hamiltonian systems defined by $\Ham_6$ and $\Ham_4$.
For this reason we will also present a number of results that
	relate properties of a generic multilinear functional $\E(f_1,\ldots,f_{2n})$, to the flow induced by the Hamiltonian $\Ham(f)=\E(f,\ldots,f)$ associated to it.



Our approach here is abstract, but we consider the abstraction justified for three reasons.
First, it is efficient.
Once we have proved, for example, $L^2$ local wellposedness for the partial differential equation induced by \eqref{eqn:3:EA},
	it will immediately imply $L^2$ local wellposedness for the two \emph{distinct} systems defined by \eqref{eqn:3:hams}.
Second, our approach clarifies which structure in the Hamiltonians \eqref{eqn:3:hams} is responsible for certain dynamics.
As a byproduct, it suggests that many of the remarkable properties of these Hamiltonian systems
	(large number of symmetries, wellposedness in many spaces, Hermite functions as stationary waves) are generic.
Third, one might expect that there are other Hamiltonian systems of mathematical or physical interest that can be cast into the framework suggested by the representations
	in \eqref{eqn:3:hams}.
Our results here would immediately give significant insight into the dynamics of such systems.



\subsection{The multilinear functional framework}

In what follows, plain Latin letters such as $E_A$, $T_A$ and $H_A$ will denote the specific multilinear functional defined by \eqref{eqn:3:EA}
	and objects associated to it.
Curly letters $\E$, $\T$, and $\Ham$ will denote a generic multilinear functional, multilinear operator and Hamiltonian respectively. 
All multilinear functionals take $2n$ arguments, are linear in the first $n$ arguments and conjugate linear in the last $n$ arguments, as in \eqref{eqn:3:EA}.

The functional properties of $E_A$ depend strongly on the matrix properties of $A$.
In the representations in \eqref{eqn:3:hams},
	the matrices involved are all isometries,
	and we will find that this structural property plays a key role in the analysis. 
We will therefore assume throughout that the matrix $A$ is an isometry.

\begin{defn}
	\label{defn:3:1}
	(i) To each matrix $A$ we associate a multilinear operator $T_A$ defined implicitly by the formula,
	\begin{equation}
		\jap{ T_A(f_1,\ldots, f_{2n-1}), g }_{L^2} = 2 \sum_{k=1}^n E_A( f_1,\ldots,f_{n+k-1},g,f_{n+k},\ldots,f_{2n-1} ).
		\label{eqn:3:defnTAimp}
	\end{equation}
	(ii) To each matrix $A$ we associate a function $H_A$ defined by $H_A(f) = E_A(f,\ldots,f)$.
\end{defn}

These definitions are motivated by the following theorem.


\begin{thm}
	\label{thm:3:EisHam}
	Suppose that a multilinear functional $\E(f_1,\ldots,f_{2n})$ has the permutation symmetry,
	\begin{equation}
		\E(f_1,\ldots,f_n,f_{n+1},\ldots,f_{2n})
			= \overline{ \E(f_{n+1},\ldots,f_{2n},f_{1},\ldots,f_{n}) }.
			\label{eqn:3:permsym}
	\end{equation}
	Then $\Ham(f)=\E(f,\ldots,f)$ is a real valued function and hence a Hamiltonian on the phase space $L^2(\R \rightarrow \C)$.
	Hamilton's equation of motion is given by $iu_t(t) = \T(u(t),\ldots,u(t))$ where the multilinear operator $\T$ is defined implicitely by
	\begin{equation}
		\jap{ \T(f_1,\ldots, f_{2n-1}), g }_{L^2} = 2 \sum_{k=1}^n \E( f_1,\ldots,f_{n+k-1},g,f_{n+k},\ldots,f_{2n-1} ).
		\label{eqn:3:defnTimp}
	\end{equation}
\end{thm}
\begin{proof}
	First, if \eqref{eqn:3:permsym} is satisfied, then
	$\Ham(f) = \E(f,\ldots,f) = \overline{\E(f,\ldots,f)} = \overline{ \Ham(f) }$, and therefore $\Ham(f)\in \R$.


	In order to find Hamilton's equation of motion corresponding to $\Ham$, we first recall the Hamiltonian phase space structure of $L^2(\R \rightarrow \C)$.
	A symplectic form on $L^2$ is given by $\omega(f,g) = -\Im \jap{f,g}_{L^2}$.
	Given a Hamiltonian $\Ham:L^2 \rightarrow \R$, the symplectic gradient $\nabla_\omega \Ham$ is defined as the unique solution of the equation
	\begin{equation}
		\omega(\nabla_\omega \Ham(f),g) = 
			\left. \frac{d}{d\epsilon} \right|_{\epsilon=0} \Ham(f+\epsilon g).
			\label{eqn:3:symgrad}
	\end{equation}
	Hamilton's equation is then $u_t = \nabla_\omega \Ham(u)$.


	In the case when $\Ham(f) = \E(f,\ldots,f)$, we have, by multilinearity,
	\begin{align}
		\left. \frac{d}{d\epsilon} \right|_{\epsilon=0} \Ham(f+\epsilon g)
		&= \left. \frac{d}{d\epsilon} \right|_{\epsilon=0} \E(f+\epsilon g,\ldots,f+\epsilon g)	\notag \\
		&= \sum_{k=1}^{2n}  \E( \manyf{k-1},g, \manyf{2n-k})
		= 2 \Re \sum_{k=1}^{n}  \E( \manyf{n+k-1},g, \manyf{2n-k} ),
		\label{eqn:3:variationR}
	\end{align}
	where in the last step we used the permutation symmetry \eqref{eqn:3:permsym}.
	On the other hand, setting,
	%$\T(f,\ldots,f) = i \nabla_w \Ham(f)$,
	\[
             i \nabla_w \Ham(f) = \T(f,\ldots,f),
             \]
	we find,
	\begin{equation}
		\omega(\nabla_\omega \Ham(f),g) 
			=  -\Im \langle i \T(f,\ldots,f),g \rangle
			=  \Re 
				\langle \T(f,\ldots,f),g \rangle.
		\label{eqn:3:variationL}
	\end{equation}
	By the definition of the symplectic gradient in \eqref{eqn:3:symgrad}, the right hand sides of \eqref{eqn:3:variationR} and \eqref{eqn:3:variationL}
		must match for all $f$ and $g$.
	By replacing $g$ by $ig$ and using conjugate linearity, we see that this equality condition holding for all $g$ actually implies that,
	\[
		\langle \T(f,\ldots,f),g \rangle
		= 2 \sum_{k=1}^{n}  \E( \manyf{n+k-1},g, \manyf{2n-k} ),
	\]
	which, in polarized from, is precisely \eqref{eqn:3:defnTimp}.

	Finally, Hamilton's equation is $i u_t =i \nabla_w H(u) =  \T(u,\ldots,u )$.
\end{proof}

For a generic isometry $A$, the functional $E_A$ does not satisfy the permutation symmetry condition \eqref{eqn:3:permsym}.
However, if we define, for example,
	\[
		\widetilde{E}_A(f_1,\ldots,f_{2n}) = \frac{1}{2} \left[ E_A(f_1,\ldots,f_{2n}) + \overline{E_A(f_{n+1},\ldots,f_{2n},f_1,\ldots,f_n}) \right],
	\]
	then $\widetilde{E}_A$ does satisfy \eqref{eqn:3:permsym}, and all the properties of $E_A$ we prove below carry over to $\widetilde{E}_A$.
	We will not be concerned with this point, because while the functionals $E_A$ do not have the permutation symmetry \eqref{eqn:3:permsym},
	the functionals $\E_6$ and $\E_4$ defined in \eqref{eqn:1:quinticE} and \eqref{eqn:1:cubicE} do.%, which are the main focus of this article, do.% satisfy \eqref{eqn:3:permsym}.
	

Before presenting general results on $E_A$, 
	we give two concrete examples.
These two examples illustrate how different isometries $A$ can give rise to very different partial differential equations $iu_t= T_A(u,\ldots,u)$.


\begin{example}
	\label{ex:3:1}
	Take $n=2$ and let $A:\R^2 \rightarrow \R^2$ be the identity matrix.
	Then,
	\[
		E_A(f_1,f_2,f_3,f_4) = \int_{\R^2} f_1(x_1) f_2(x_2) \overline{ f_3(x_1) f_4(x_2) } dx = \jap{f_1,f_3}_{L^2} \jap{f_2,f_4}_{L^2},
	\]
	and hence $H_A(f) = \| f \|_{L^2}^4$.
	We calculate,
	\begin{align*}
		T_A(f_1,f_2,f_3)(y) &= 2\left[ 
			\int_\R f_1(x_1) \left[f_2(x_2) \overline{ f_3(x_2) }\right] \delta_{y=x_1} dx	+
			\int_\R \left[ f_1(x_1) \overline{ f_3(x_1) }\right] f_2(x_2) \delta_{y=x_2} dx
		\right]		\\
		&= 2 f_1(y) \jap{f_2,f_3}_{L^2} + 2 f_2(y) \jap{f_1,f_3}_{L^2}.
	\end{align*}
	Hamilton's equation is then
	$
		i u_t = T_A(u,u,u) = 4 u \| u \|_{L^2}^2,
	$
	which has a unique solution for initial data $u_0\in L^2$ given by $u(x,t) = e^{4i\|u_0\|_{L^2}^2 t} u_0(x)$.
\end{example}


\begin{example}
	\label{ex:3:2}
	Take $n=2$ again, and 
	let $A= \frac{1}{\sqrt{2}} \begin{pmatrix} 1 & -1 \\ 1 & 1  \end{pmatrix}$ be the rotation of $\R^2$ by $\pi/4$ radians.
	Then,
	\[
		E_A(f_1,f_2,f_3,f_4) = \int_{\R^2} 
			f_1\left( \frac{x_1-x_2}{\sqrt{2}} \right) f_2\left( \frac{x_1+x_2}{\sqrt{2}} \right) \overline{ f_3(x_1) f_4(x_2) } dx.
	\]
	and,
	\begin{align}
		T_A(&f_1,f_2,f_3)(y) \notag \\&= 2 \left[ 
			\int_\R 
			f_1\left( \frac{y-s}{\sqrt{2}} \right) f_2\left( \frac{y+s}{\sqrt{2}} \right) \overline{ f_3(s) } ds
			+ \int_\R 
			f_1\left( \frac{s-y}{\sqrt{2}} \right) f_2\left( \frac{s+y}{\sqrt{2}} \right) \overline{ f_3(s) } ds.
		\right]
		\label{eqn:3:ex2TA}
	\end{align}
	In this case it is not clear that the general solution of the equation $iu_t = T_A(u,u,u)$ can be written explicitly.
	However it is still possible to determine many properties of the flow.
	For example,
		one may verify by substitution that, for any $\alpha>0$, the functions
		$u(x,t) = e^{i \sqrt{ 8\pi/\alpha }  t} e^{-\alpha x^2}$ and $u(x,t)=xe^{-\alpha x^2}$, are explicit solutions of $iu_t =T_A(u,u,u)$
		(the second solution does not depend on time).
	These solutions were both produced using Corollary \ref{thm:3:stationary} below.
\end{example}






\subsection{Symmetries of the functional and associated conservation laws}


In this subsection we uncover some of the rich symmetry structure of the functional $E_A$.
We recall that $A$ is assumed to be an isometry throughout.
\begin{thm}
	\label{thm:3:fourier}
	The functional $E_A$ is invariant under the Fourier transform, that is,
	\begin{equation}
		E_A( \ft_1,\ldots,\ft_{2n}) = E_A(f_1,\ldots,f_{2n}).
		\label{eqn:3:Fouriersym}
	\end{equation}
	It follows that ${ T_A( \ft_1,\ldots,\ft_{2n-1})) }(\xi) = \widehat{T_A}( f_1,\ldots, f_{2n-1} )(\xi)$.
\end{thm}




\begin{proof}
Because $A$ is an isometry, we have $\langle \xi, Ax \rangle = \langle A^{-1} \xi, x \rangle$
	for all $\xi,x \in \R^n$.
Now calculating,
\begin{align*}
	E_A(\ft_1,\ldots,\ft_{2n})	
	&= \int_{\R^n} \prod_{k=1}^n \ft_k( (Ax)_k ) \overline{\ft_{n+k}( x_k )} dx		\\&
				= \frac{1}{(2\pi)^n} \int_{\R^n}  \prod_{k=1}^n 
					\left( \int_{\R} e^{-i\xi_k (Ax)_k } f_k(\xi_k) d\xi_k \right)
					\left( \int_{\R} e^{i\nu_k x_k } \of_{n+k}(\nu_k) d\nu_k \right)
				dx		\\
		&%= \frac{1}{(2\pi)^n}   \int_{\R^n} \int_{\R^{2n}} e^{ -i \langle \xi, Ax\rangle + i \langle \nu, x \rangle }
		%	\prod_{k=1}^n f(\xi_k) \of(\nu_k) d\xi d\nu dx		%\\&
		= \frac{1}{(2\pi)^n}   \int_{\R^n} \int_{\R^{2n}} e^{ -i \langle A^{-1}\xi -  \nu, x \rangle }
			\prod_{k=1}^n f_k(\xi_k) \of_{n+k}(\nu_k) d\xi d\nu dx,
\end{align*}
	where in the last line we have used $\jap{\xi,Ax}+\jap{\nu,x}=\jap{A^{-1}\xi-\nu,x}$.
	We first change variables $y(\xi)= A^{-1}\xi - \nu$, or $\xi(y) = Ay+ A\nu$.
The determinant of this change of variables is 1 because $A$ is an isometry.
Performing the change of variables then gives the required identity,
	\begin{align*}
	E_A(\ft_1,\ldots,\ft_{2n})	
		&= \frac{1}{(2\pi)^n}   \int_{\R^n} \int_{\R^{2n}} e^{ -i \langle y, x \rangle }
			\prod_{k=1}^n f_k(A\nu_k + Ay) \of_{n+k}(\nu_k) dy d\nu dx	\\
			&=
		  \int_{\R^n} \int_{\R^{2n}} 
			\prod_{k=1}^n f_k((A\nu)_k) \of_{n+k}(\nu_k) d\nu  = E_A(f_1,\ldots,f_{2n}),
	\end{align*}
	where in the second equality we used the Fourier inversion identity \eqref{eqn:1:fourierinv} with $a=1$.


For the operator statement, let $g$ be an arbitrary element of $L^2$.
Using the definition of $T_A$ in \eqref{eqn:3:defnTAimp} we have,
	\begin{align}
		\langle \widehat{ T_A }(f_1,\ldots,f_{2n-1}) , \widehat{g} \rangle	&=
	\langle { T_A }(f_1,\ldots,f_{2n-1}) , {g} \rangle	=
	2 \sum_{k=1}^n E_A( f_1,\ldots,f_{n+k-1},g,f_{n+k},\ldots,f_{2n-1} ) 	\notag \\
		&= 2 \sum_{k=1}^n E_A( \ft_1,\ldots,\ft_{n+k-1},\hat{g},\ft_{n+k},\ldots,\ft_{2n-1} )   \notag \\
                &=
		\langle T_A(\ft_1,\ldots,\ft_{2n-1}), \widehat{g} \rangle.
		\label{eqn:3:fourierT}
	\end{align}
The operator identity follows.
\end{proof}







\begin{thm}
	\label{thm:3:symmetries}
	\label{thm:3:symE}
	The functional $E_A$ is invariant under the following actions (for any $\lambda$):
	\begin{enumerate}[label=(\roman*)]
		\item	Modulation: $f_k \mapsto e^{i\lambda} f_k$.
		\item	$L^2$ scaling: $f_k(x) \mapsto \lambda^{1/2} f_k(\lambda x)$.
		\item	Quadratic modulation: $f_k \mapsto e^{i\lambda |x|^2} f_k$.
		\item	\Sch{} group: $f_k \mapsto e^{i\lambda \Delta} f_k$.
		\item	\Sch{} with harmonic trapping group: $f_k \mapsto e^{i\lambda H} f_k$, where $H=-\Delta+|x|^2$.
	\end{enumerate}	
	If, in addition, $A$ satisfies  $Ae=e$, where $e=(1,\ldots,1) \in \R^n$, then $E_A$ is invariant under the following actions (for any $\lambda$):
	\begin{enumerate}[resume,label=(\roman*)]
		\item	Linear modulation: $f_k \mapsto e^{i\lambda x  } f_k$.
		\item	Translation: $f_k \mapsto f_k(\cdot+\lambda)$.
	\end{enumerate}	
\end{thm}
\begin{proof}


\begin{enumerate}[label=(\roman*)]
	\item
	We have,
	$$
		E_A( e^{i\lambda} f_1,\ldots,e^{i\lambda} f_{2n} ) 
			= \int_{ \R^n } \prod_{k=1}^n e^{ i\lambda} f_1( (Ax)_k ) e^{-i\lambda} \of_{2n}( x_k ) dx 
			= E_A(f_1,\ldots,f_{2n}).
	$$
	\item

	 Let $f_k^\lambda(x) = \lambda^{1/2} f_k(\lambda x)$.
	We write out $E_A$ and perform the change of variables 
		$y = \lambda x$ (with $dy = \lambda^n dx$) to find,
	\begin{align*}
		E_A(f_1^\lambda,\ldots,f_{2n}^\lambda)
			&= \lambda^{n} \int_{ \R^n } \prod_{k=1}^n f_k( \lambda (Ax)_k )  \of_{n+k}( \lambda x_k ) dx   \\
			&=  \int_{ \R^n } \prod_{k=1}^n f( (Ay)_k )\of(  x_k ) dx 
			=  E_A(f_1,\ldots,f_{2n}).
	\end{align*}

	\item
		Because $A$ is an isometry,
		$\nrm{Ax}^2=\nrm{x}^2$ for all $x \in \R^n$.
	Using this, we have,
	\begin{align*}
		E_A( e^{i\lambda |x|^2} f_1,\ldots, e^{i\lambda |x|^2} f_{2n} ) 
			&= \int_{ \R^n } \prod_{k=1}^n e^{ i\lambda |(Ax)_k|^2 } f_k( (Ax)_k ) e^{-i\lambda |x_k|^2} \of_{n+k}( x_k ) dx 	\\
			&= \int_{ \R^n } e^{i \lambda |Ax|^2} e^{-i\lambda |x|^2 } \prod_{k=1}^n f_k( (Ax)_k ) \of_{n+k}( x_k ) dx  \\
			&= E_A(f_1,\ldots,f_{2n}).
	\end{align*}

\item
	Using the previous part and the invariance of the Hamiltonian under the Fourier transform, we find,
	\begin{align*}
		E_A( e^{i\lambda \Delta} f_1,\ldots, e^{i\lambda \Delta} f_{2n} ) 
                &=
		E_A( e^{-i\lambda |x|^2} \ft_1,\ldots, e^{-i\lambda |x|^2} \ft_{2n} )\\ 
			&= E_A(\ft_1,\ldots,\ft_{2n})    
		    = E_A(f_1,\ldots,f_{2n}).
	\end{align*}

\item	In this part we use $t$ instead of $\lambda$, and show invariance of the functional under $e^{itH}$.

	First, we note that if $n$ is an integer then $e^{i(\pi/2+n\pi)H} f = \ft$ (from, for instance, the Mehler formula \eqref{eqn:2:mehler}).
	The $t = \pi/2+n\pi$ case thus follows from Theorem \ref{thm:3:fourier}.

	If $t \neq \pi/2+n\pi$ then we may represent $e^{itH}f$ using the \emph{lens transform} \cite{Tao2009}.
		This transform relates 
		solutions of the free linear \Sch{} to the linear \Sch{} equation with harmonic trapping.
	Precisely, there holds,
		\begin{equation}
		(e^{itH}f_k)(x) =
			\frac{1}{ \sqrt{ \cos(2t) } } (e^{i(\tan(2t)/2)\Delta}f_k) \left( \frac{ x}{\cos(2t)} \right) e^{ix^2 \tan(2t)/2} .
			\label{eqn:3:lenstransform}
		\end{equation}
	We substitute this expression into the functional.
		Using in turn the symmetries (iii) (with $\lambda = \tan(2t)/2$), (ii) (with $\lambda = 1/\cos(2t)$), and (iv) (with $\lambda = \tan(2t)/2)$, we determine that,
	\begin{align*}
		E_A&( e^{ i t H } f_1, \ldots, e^{i t H} f_{2n} ) \\
			&=
			E_A \left(
				\frac{1}{ \sqrt{ \cos(2t) } } (e^{i(\tan(2t)/2)\Delta}f_1) \left( \frac{ x}{\cos(2t)} \right),\right.   \\
                                & \left. \hspace{2cm}\ldots,
				\frac{1}{ \sqrt{ \cos(2t) } } (e^{i(\tan(2t)/2)\Delta}f_{2n}) \left( \frac{ x}{\cos(2t)} \right) \right)	\\
			&=
			E_A \left(
				(e^{i(\tan(2t)/2)\Delta}f_1) \left( x \right),\ldots,
				(e^{i(\tan(2t)/2)\Delta}f_{2n}) \left( x  \right) \right) = E_A( f_1,\ldots,f_{2n}).
	\end{align*}

\item
	In these last two parts we assume that, in addition to being an isometry, the matrix $A$ also satisfies
		$Ae=e$ for $e=(1,\ldots,1)\in \R^n$.
	We then have,
	\begin{align*}
		E_A( e^{i\lambda x} f_1,\ldots, e^{i\lambda x}f_{2n} ) 
			&= \int_{ \R^n } \prod_{k=1}^n e^{ i\lambda (Ax)_k } f_k( (Ax)_k ) e^{-i\lambda x_k} \of_{n+k}( x_k ) dx	\\
			&= \int_{ \R^n } e^{i\lambda \langle Ax, e \rangle } e^{-\lambda \langle x, e \rangle} \prod_{k=1}^n  f_k( (Ax)_k ) \of_{n+k}( x_k ) dx     \\
			&= E_A(f_1,\ldots,f_{2n}).
	\end{align*}
	where in the last step we used $\langle Ax,e\rangle= \langle x, A^{-1}e \rangle=\langle x,e\rangle$.

\item
	This follows immediately from the previous part and the invariance of the functional  under the Fourier transform, as in item (iv),
		noting that the Fourier transform takes
		$x\mapsto e^{i\lambda x  } f(x)$ to 
		$\xi \mapsto \ft(\xi+\lambda)$.
	\end{enumerate}	
\end{proof}


The symmetries of the functional $E_A$ lead directly to commutator identities for the operator $T_A$.

\begin{corr}
	\label{thm:3:commuter}
	We have the following commuter identities,
	\begin{align}
		e^{i\lambda Q} T_A(f_1,\ldots,f_{2n-1}) &= T_A(e^{i \lambda Q} f_1,\ldots,e^{i \lambda Q} f_{2n-1})		\label{eqn:3:TAcomm1} \\
		Q T_A(f_1,\ldots,f_{2n-1}) &= \sum_{k=1}^n T_A(f_1,\ldots,f_{k-1},Qf_k,f_{k+1},\ldots f_{2n-1})	\notag \\
			&\hspace{1cm}- \sum_{k=n+1}^{2n-1} T_A(f_1,\ldots,f_{k-1},Qf_k,f_{k+1},\ldots f_{2n-1}) \label{eqn:3:TAcomm2} 
	\end{align}
	where $Q$ is any of the following operators.
	\begin{enumerate}
		\item For a generic isometry $A$, $Q=1$, $Q = x^2$, $Q=\Delta$ and $Q=H$.
		\item If in addition $Ae=e$, where $e=(1,\ldots,1)$, $Q = x$, $Q=i d/dx$.
	\end{enumerate}
\end{corr}
\begin{proof}
	For each of the operators $Q$, the flow map $e^{i\lambda Q}$ is an isometry of $L^2$ for all $\lambda$, and,
	\[
		E_A( e^{i\lambda Q} f_1,\ldots, e^{i\lambda Q} f_{2n} ) 
		= E_A( f_1,\ldots, f_{2n} ) ,
	\]
	from Theorem \ref{thm:3:symmetries}.
	For each $g \in L^2$, we thus have,
	\begin{align*}
		\langle e^{i\lambda Q} &T_A(f_1,\ldots,f_{2n-1}),g \rangle_{L^2} \\
			&= \langle  T_A(f_1,\ldots,f_{2n-1}),e^{-i\lambda Q} g \rangle_{L^2} 	\\
			&= 2 \sum_{k=1}^{n} E_A\left(  f_1,\ldots, f_{n+k-1}, e^{-i\lambda Q} g, f_{n+k},\ldots, f_{2n-1},  \right)\\
			&= 2 \sum_{k=1}^{n} E_A\left( e^{i \lambda Q} f_1,\ldots, e^{i \lambda Q} f_{n+k-1}, g,
				e^{i \lambda Q} f_{n+k},\ldots,e^{i \lambda Q} f_{2n-1},  \right)\\
			&= \langle T_A(e^{i \lambda Q} f_1,\ldots,e^{i \lambda Q} f_{2n-1}), g\rangle_{L^2},
	\end{align*}
	which gives \eqref{eqn:3:TAcomm1}.
	To get \eqref{eqn:3:TAcomm2}, differentiate \eqref{eqn:3:TAcomm1} with respect to $\lambda$ and set $\lambda=0$. 
\end{proof}


In Hamiltonian mechanics, the primary purpose of finding symmetries is to determine conservation laws.
These two concepts are linked through Noether's theorem.
We have seen, in Theorem \ref{thm:3:EisHam}, that in the present context if a functional $\E$ satisfies the permutation symmetry
	\eqref{eqn:3:permsym}, then the functional gives rise to a Hamiltonian $\Ham$ and Hamilton's equation of motion is $iu_t = \T(u,\ldots,u)$.
With this Hamiltonian structure, a version of Noether's Theorem applies. 

\begin{thm}[Noether's Theorem]
	\label{thm:3:noether}
	Let $\E$ be a multilinear functional that satisfies the permutation symmetry \eqref{eqn:3:permsym}.
	Suppose that $Q$ is a self-adjoint operator on $L^2$ such that
	\begin{equation}
		\E( e^{i\lambda Q}f_1,\ldots, e^{i\lambda Q} f_{2n})=
		\E( f_1,\ldots, f_{2n}).
		\label{eqn:3:Econserved0}
	\end{equation}
	Then the quantity $\jap{ Qf, f}_{L^2}$ is conserved by the Hamiltonian flow of $\Ham(f)=\E(f,\ldots,f)$.
\end{thm}


\begin{proof}
	We first show that $\jap{\T(f,\ldots,f),Qf} \in \R$.
	Differentiating equation \eqref{eqn:3:Econserved0} with respect to $\lambda$ and setting $\lambda=0$ gives,
	\begin{equation}
		\sum_{k=1}^n \E(\manyf{k-1}, Qf, \manyf{2n-k} ) = \sum_{k=1}^n \E( \manyf{n+k-1},Qf,\manyf{n-k});
		\label{eqn:3:Econserved1}
	\end{equation}
	the sign being determined by the linearity or conjugate linearity of each component. 
	Now using the permutation symmetry \eqref{eqn:3:permsym} followed by \eqref{eqn:3:Econserved1} gives,
	\begin{align*}
		\overline{ \jap{ \T(f,\ldots,f),Qf } }
		&= 2\sum_{k=1}^n \overline{ \E( \manyf{n+k-1},Qf,\manyf{n-k}) } 	=2 \sum_{k=1}^n \E(\manyf{k-1}, Qf, \manyf{2n-k} ) 	\\
		&=2 \sum_{k=1}^n { \E( \manyf{n+k-1},Qf,\manyf{n-k}) }
		= \jap{ \T(f,\ldots,f),Qf },
		\label{eqn:3:Econserved1}
	\end{align*}
	which shows that $\jap{ \T(f,\ldots,f), Qf }$ is real.
	Then, if $if_t= \T(f,\ldots,f)$, we have
	\begin{align*}
		\frac{d}{dt} \jap{Qf,f} 
			&= i \left[
			\jap{ Q\T(f,\ldots,f),f }
			-\jap{ Qf, \T(f,\ldots,f) }
			\right]	\\
			&= i \left[
			\jap{ \T(f,\ldots,f),Qf }
			-\jap{ Qf,\T(f,\ldots,f) }
			\right] = 2i \Im \jap{ \T(f,\ldots,f), Qf } = 0,
	\end{align*}
	so $\jap{Qf,f}$ is constant.
\end{proof}


Table \ref{tab:1} summarizes the relationships between 
	the symmetries of $E_A$ described in Theorem \ref{thm:3:symmetries},
	the associated commuting operators in Corrolary \ref{thm:3:commuter},
	and the conserved quantities given by Noether's Theorem.
As discussed previously, the functional $E_A$ does not automatically satisfy the permutation symmetry \eqref{eqn:3:permsym} so Noether's Theorem does not apply directly;
	however, the Hamiltonian systems defined by $\Ham_6$ and $\Ham_4$ do satisfy \eqref{eqn:3:permsym} and so will have a number of these conserved quantities
	as a consequence of symmetries induced by Theorem \ref{thm:3:symmetries}.

\begin{table}

\begin{center}
	\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|ccc|}\hline
		Symmetry $e^{i\lambda Q}$ of $\E$	&Operator $Q$ commuting with $\T$ 	&Conserved quantity $\jap{Qf,f}$			\\ \hline
		$f\mapsto e^{i\lambda}f$		&$1$					&$\int_\R |f(x)|^2 dx$					\\
		$f\mapsto f_\lambda$			&					&$\int_\R \left[ i xf'(x)+f(x) \right] \of(x)  dx$	\\
		$f\mapsto e^{i\lambda |x|^2}f$		&$x^2$					&$\int_\R |xf(x)|^2 dx$					\\
		$f\mapsto e^{i\lambda \Delta}f$		&$\Delta$				&$\int_\R |f'(x)|^2 dx$	 				\\
		$f\mapsto e^{i\lambda \HO}f$		&$H$					&$\int_\R |x f(x)|^2 + |f'(x)|^2 dx$ 			\\
		$f\mapsto e^{i\lambda x}f$		&$x$					&$\int_\R x|f(x)|^2 dx$					\\
		$f\mapsto f(\cdot+\lambda)$		&$id/dx$				&$\int_\R i f'(x) \of(x)   dx$				\\ \hline
	\end{tabular}
\end{center}
\caption{Relationship between the symmetries of $\E$ and the conserved quantites 
of the Hamiltonian flow, as given by Noether's Theorem.}
\label{tab:1}
\end{table}


\subsection{Boundedness and wellposedness}
In this subsection we establish an $L^2$ bound on $E_A$,
	%the bound
	%$|E_A(f_1,\ldots,f_{2n})| \leq \| f_1 \|_{L^2} \cdots \| f_{2n} \|_{L^2}$
and bounds of the form,
\begin{equation}
	\| T_A(f_1,\ldots,f_{2n-1}) \|_X \leq C \| f_1 \|_X \cdots \| f_{2n-1} \|_X,
\end{equation}
for $X=L^2$, $X=L^{2,\sigma}$ and $X=H^\sigma$.
We will then show how these bounds imply local existence of solutions to
	Hamilton's equation $i u_t = T_A(u,\ldots,u)$ in the space $X$.
By employing some of the conservation laws derived in the last section,
	it is possible to establish global existence in $L^2$ and other spaces for certain functionals.

\begin{thm}
	\label{thm:3:L2bound}
	There holds the bound,
	\begin{equation}
		| E_A(f_1,\ldots,f_{2n}) | \leq 
			\prod_{k=1}^{2n} \| f_k \|_{L^2}.
		\label{eqn:3:boundonEA}
	\end{equation}
	In particular we have $H_A(f) \leq \| f \|_{L^2}^{2n}$.
	Both of these bounds are sharp.
\end{thm}

\begin{proof}
	The proof involves one use of the \CS{} inequality.
	We have,
	\begin{align*}
		| E_A(f_1,\ldots,f_{2n}) | 
			&= 	\left| \int_{ \R^n } \prod_{k=1}^n f_k( (Ax)_k ) \of_{n+k}( x_k ) dx \right|	\\
			&\leq 	
				\left( \int_{ \R^n } \prod_{k=1}^n |f_k( (Ax)_k )|^2 dx \right)^{1/2}
				\left( \int_{ \R^n } \prod_{k=1}^n |f_{n+k}( x_k )|^2 dx \right)^{1/2}.
	\end{align*}
	In the first integral we perform the change of variables $y=Ax$.
	Because $A$ is an isometry, the determinant of this change of variables is 1, and so by Fubini's Theorem,
	\begin{align*}
		| E_A(f_1,\ldots,f_{2n}) | 
			&\leq 	
				\left( \int_{ \R^n } \prod_{k=1}^n |f_k( y_k )|^2 dy \right)^{1/2}
				\left( \int_{ \R^n } \prod_{k=1}^n |f_{n+k}( x_k )|^2 dx \right)^{1/2}	%\\&
			%=	
			%	\left(  \prod_{k=1}^n \int_{\R} |f_k( y_k )|^2 dy_k \right)^{1/2}
			%	\left( \prod_{k=1}^n \int_{ \R } |f_{n+k}( x_k )|^2 dx_k \right)^{1/2}
			=\prod_{k=1}^{2n} \| f_k \|_{L^2},
	\end{align*}
	which is the bound for $E_A$.
	Setting $f_k=f$ for all $k$ gives the bound $H_A(f) \leq \| f \|_{L^2}^2$.

	From the \CS{} inequality, we have the equality condition,
	\begin{equation}
		\prod_{k=1}^n f_k( (Ax)_k ) = \prod_{k=1}^n f_{n+k}( x_k ).
		\label{eqn:3:cseq}
	\end{equation}
	By assumption, $A$ is an isometry, so that $ \sum_{k=1}^n |(Ax)_k|^2 = \nrm{Ax}^2 = \nrm{x}^2 = \sum_{k=1}^n |x_k|^2$.
	This immediately gives that the Gaussian $G(x) = e^{-\alpha x^2}$ satisfies the equality condition \eqref{eqn:3:cseq},
	and hence that $H(G)=\|G\|_{L^2}^{2n}$.
	The inequality \eqref{eqn:3:boundonEA} is thus sharp.
\end{proof}


In a later subsection we discuss the classification of all functions $\{ f_k \}_{k=1}^{2n}$ that saturate the multilinear functional inequality \eqref{eqn:3:boundonEA}.
The two examples on page \pageref{eqn:3:ex2TA} show that, in general, such a classification will depend on the matrix properties of $A$.
In Example \ref{ex:3:1},  $H_A(f) = \| f \|_{L^2}^4$, and so the bound $H_A(f) \leq \| f \|_{L^2}^4$ in Theorem \ref{thm:3:L2bound} is \emph{always} equality.
This is not the case in Example \ref{ex:3:2}.
In Theorem \ref{thm:3:maxH}, we will find that if $A$ is not a signed permutation matrix -- namely that there is at least one basis element $e_k$
	such that $Ae_k$ is a linear sum of at least two other $e_j$ basis elements --
	then the equality $H_A(f) = \| f \|_{L^2}^{2k}$ holds only if $f$ is a Gaussian.

In the meantime, we use the inequality \eqref{eqn:3:boundonEA} to establish bounds for the multilinear operator $T_A$.

\begin{corr}
	\label{thm:3:Tbound}
	There holds the bound,
	\[
		\|T_A(f_1,\ldots,f_{2n-1})\|_{X} \leq C_n  \prod_{k=1}^{2n-1}\| f_k \|_{X}^{2n-1}
	\]
	for the following spaces.
	\begin{enumerate}[label=(\roman*)]
		\item $X=L^2$ with $C_n=2n$;
		\item $X=L^{2,\sigma}$, for any $\sigma \geq 0$ with $C_n = 2n^{2+\sigma}$.
		\item $X=H^{\sigma}$, for any $\sigma \geq 0$ with $C_n = 2n^{2+\sigma}$.
	\end{enumerate}
\end{corr}

It is important that the boundedness constant $C_n$ is independent of $A$.
This implies that if we have a composite Hamiltonian of the form,
\[
	\int_\Omega \phi(\lambda) H_{A(\lambda)}(f) d\lambda,
\]
then the associated operator will be bounded once $\phi$ is integrable.
This is precisely how Corollary \ref{thm:3:Tbound} will be applied to the Hamiltonian systems $\Ham_6$ and $\Ham_4$.


\begin{proof}
	(i)
	We argue by duality using the implicit representation \eqref{eqn:3:defnTAimp}.
	By the bound on $E_A$ from Theorem \ref{thm:3:L2bound} we have,
	\begin{align*}
		|\langle T_A(f_1,\ldots,f_{2n-1}), g \rangle_{L^2}|	
			&\leq 2 \sum_{k=n+1}^{2n} |E_A( f_1,\ldots,f_{n+m-1},g,f_{n+m},\ldots, f_{2n-1})|	\\
			&\leq 2 \sum_{k=n+1}^{2n} \prod_{k=1}^{2n-1} \| f_k \|_{L^2} 	\| g \|_{L^2} 
			= \left( 2n  \prod_{k=1}^{2n-1} \| f_k \|_{L^2} \right) \| g \|_{L^2}.	
	\end{align*}
	This gives the result for $X=L^2$.


	(ii)
	Fix $x \in \R^n$.
	Because $A$ is an isometry we have, for every $m$,
	$
		|x_m|^2 \leq \nrm{x}^2 = \nrm{Ax}^2 = \sum_{k=1}^n |(Ax)_k|^2.
	$
	Therefore, for fixed $m$, there is an integer $l$ such that $|x_m|^2 \leq n | (Ax)_l |^2$.
        With $\langle\rangle$ denoting the Japanese bracket,
        we then have $\langle x_m \rangle \leq n \jap{ (Ax)_l }$ and so,
	\[
		\jap{ x_m } \leq n \left( \prod_{k=1, k\neq m}^n \jap{ (Ax)_k) } \jap{ x_k } \right) \jap{ (Ax)_m},
	\]
	because in all cases $\jap{t} \geq 1$.
	In terms of the functional $E_A$, this gives,
	\begin{equation}
		\begin{split}
			E_A(|f_1|,\ldots,|f_{k-1}|,&\jap{t}^\sigma |f_k|, |f_{k-1}|, \ldots, |f_{2n}| ) \\
			&\leq n^\sigma	E_A(\jap{t}^\sigma |f_1|,\ldots, \jap{t}^\sigma |f_{k-1}|, |f_k|, \jap{t}^\sigma |f_{k-1}|, \ldots, \jap{t}^\sigma |f_{2n}| ).
		\end{split}
		\label{eqn:3:weighttrans}
	\end{equation}

	Now applying this to $T_A$,  we have,
	\begin{align*}
		\langle T_A(f_1,&\ldots,f_{2n-1}), g \rangle_{L^{2,\sigma}} \\
			&=
			\langle T_A(f_1,\ldots,f_{2n-1}), \jap{t}^{2\sigma}  g \rangle_{L^{2}}	\\
			&= 2n \sum_{k=n+1}^{2n} E_A( f_1,\ldots,f_{k-1}, \jap{t}^{2\sigma} g,f_k,\ldots, f_{2n-1})	\\
			&\leq 2 n^{1+\sigma} \sum_{k=n+1}^{2n} E_A( \jap{t}^\sigma |f_1|,\ldots, \jap{t}^\sigma |f_{k-1}|, \jap{t}^{\sigma} |g|, \jap{t}^\sigma |f_k|,\ldots, \jap{t}^\sigma |f_{2n-1}|)	\\
			&\leq \left( 2 n^{2+\sigma} \prod_{k=1}^{2n-1} \| f_{k} \|_{L^{2,\sigma}} \right)
				\| g \|_{L^{2,\sigma}} ,
	\end{align*}
	which gives the result for $X=L^{2,\sigma}$.

	(iii) This follows from (ii) using the invariance of the operator $T_A$ under the Fourier transform.
\end{proof}



The next proposition shows that, in general, bounds of the form determined in the previous proposition imply local wellposedness.


\begin{prop}
	\label{thm:3:wellposedness}
	Suppose that $\T:X^m \rightarrow X$ is a multilinear operator that is bounded on a
		Banach space $X$; that is,
	\[
		\| \T(f_1,\ldots,f_{m})\|_X\leq C_\T \prod_{k=1}^m \|f_k\|_X
	\]
	for some $C_\T$.
	Set $\T(f)=\T(f,\ldots,f)$.
	For every $f_0\in X$ there is a $T>0$ and unique local solution to
	the Cauchy problem for Hamiltonian's equation,
	\begin{equation}
		\begin{split}
			if_t &= \T(f),		\\
			f(t=0) &= f_0,
		\end{split}
		\label{eqn:3:cauchy}
	\end{equation}
	in the space $L^\infty ([0,T],X)$.
	The time of existence $T$ depends only on $\|f_0\|_X$.

\end{prop}


\begin{proof}
	The Duhamel formulation of the Cauchy problem \eqref{eqn:3:cauchy} is
	\[
		f(t) := R(f(t)) = f_0 + \int_0^t \T(f(s))ds.
	\]
	To prove local existence we will show that there is a $T=T(\|f_0\|_X)$ such that the operator $R$ is a contraction on $Y_T = L^\infty({[0,T]},X)$.
	The proposition then follows from Banach's Fixed Point Theorem.

	We first have the bound
	\begin{equation}
		\| R(f(t)) \|_X 
			\leq \| f_0 \|_X + \int_0^t \| \T(f(s)) \|_X ds 	
			\leq \| f_0 \|_X + C_\T\int_0^t \| f(s) \|_X^{m} ds 
			\leq \| f_0 \|_X + t C_\T \| f \|_{Y_t}^{m} .
		\label{eqn:3:fixedpoint1}
	\end{equation}

	Next we have
		$\| R(f_1(t)) - R(f_2(t)) \|_X 
			\leq  \int_0^t \| \T(f_1(s)) - \T(f_2(s))  \|_X ds.$
			To evaluate the right hand side, we use multilinearity to write,
	\begin{align*}
		\T(f_1(s)) - \T(f_2(s))
		&= \T(f_1,\ldots,f_1) - \T(f_2,\ldots,f_2)	%\\&
		= \sum_{k=1}^{m} \T ( \manys{f_1}{k-1} , f_1 - f_2, \manys{f_2}{m-k} ).
	\end{align*}
	This equality gives,
	\begin{align*}
		\| \T(f_1(s)) - \T(f_2(s)) \|_X
		&\leq C_\T \sum_{k=1}^{m-1} \| f_1 \|_X^{k-1} \|f_1-f_2 \|_X \| f_2 \|_X^{m-k}	\\
		&\leq\|f_1-f_2 \|_X  (m-1) C_\T \left[ \| f_1 \|_X^{m-1} +  \| f_2 \|_X^{m-1} \right],
	\end{align*}
	and then,
	\begin{equation}
		\| R(f_1(t)) - R(f_2(t)) \|_{Y_t}
			\leq  \|f_1-f_2 \|_{Y_t} \left( t (m-1) C_\T \left[ \| f_1 \|_{Y_t}^{m-2} +  \| f_2 \|_{Y_t}^{m-2} \right] \right).
		\label{eqn:3:fixedpoint2}
	\end{equation}

	From \eqref{eqn:3:fixedpoint1} and \eqref{eqn:3:fixedpoint2} it follows that for any $M>\|f_0\|_X$ we may choose $T$ such that
	$R: B_{Y_T}(0,M) \rightarrow B_{Y_T}(0,M)$ and $R$ a contraction on this space.
\end{proof}

It is key in the proposition that the local time of existence depends only on $\|f_0\|_X$.
This enables one to pair the local wellposedness result with a conservation law in the previous subsection to get global wellposedness.
We will do precisely this to prove global wellposedness in $L^2$ of solutions to the Hamiltonian systems $\Ham_6$ and $\Ham_4$. % in sections 4 and 5 respectively.


\subsection{The functional in the basis of Hermite functions}

The symmetry of the functional under the action $e^{itH}$ implies interesting explicit relationships between $E_A$, $T_A$ and the Hermite functions $\{\phi_n\}_{n=0}^\infty$.
\begin{thm}
	\label{thm:3:hermite}
	If $ \sum_{k=1}^n m_k - \sum_{k=n+1}^{2n} m_k \neq 0$, then $E_A( \phi_{m_1},\ldots, \phi_{m_{2n}}) = 0$.
	This implies that,
	\begin{equation}
		T_A(\phi_{m_1},\ldots,\phi_{m_{2n-1}}) = C \phi_l,
		\label{eqn:3:TAinhermite}
	\end{equation}
	for some constant $C$
	where $l = \sum_{k=1}^n m_k - \sum_{k=n+1}^{2n-1} m_k$.
	(We understand that if $l<0$ then $\phi_l:=0$.)
\end{thm}


\begin{proof}
	By the symmetry under the action $e^{itH}$, we have
	\begin{align*}
		E_A( \phi_{m_1},\ldots, \phi_{m_{2n}}) &=
		E_A( e^{itH} \phi_{m_1},\ldots, e^{itH} \phi_{m_{2n}}) \\&=
		E_A( e^{it(2m_1+1)} \phi_{m_1},\ldots, e^{it ( 2 m_{2n}+1) } \phi_{m_{2n}}) \\&=
		e^{it2L}
		E_A( \phi_{m_1},\ldots, \phi_{m_{2n}}) 
	\end{align*}
	where $L= \sum_{k=1}^n m_k - \sum_{k=n+1}^{2n} m_k$.
	If $L\neq0$, as in the statement of the theorem, then necessarily the $E_A$ term here is 0.

	Next, let $m_1,\ldots,m_{2n-1}$ be given, and fix
		$p \neq \sum_{k=1}^n m_k - \sum_{k=n+1}^{2n-1} m_k $.
	We have,	% the implicit representation of $T_A$ in \eqref{eqn:3:defnTAimp} we have,
	\[
		\jap{ T_A(\phi_{m_1},\ldots,\phi_{m_{2n-1}}), \phi_p }_{L^2}
		= 2 \sum_{k=1}^n
			E_A( \phi_{m_1},\ldots, \phi_{m_{n+k-1}}, \phi_p ,\phi_{m_{n+k}}, \ldots, \phi_{m_{2n}})  = 0,
	\]
	by the previous part and because 
	$p \neq \sum_{k=1}^n m_k - \sum_{k=n+1}^{2n-1} m_k $.
	The function $T_A(\phi_{m_1},\ldots,\phi_{m_{2n-}})$ is thus orthogonal to $\phi_p$ for all such $p$.
	Because the Hermite functions are an orthonormal basis of $L^2$, we must have \eqref{eqn:3:TAinhermite}.
\end{proof}


\begin{corr}
	\label{thm:3:stationary}
	Set $\omega_n = 2n H_A(\phi_n)$.
	Then $u(t,x) = e^{it\omega_n} \phi_n(x)$ is a stationary wave solution of $iu_t = T_A(u,\ldots,u)$.
\end{corr}

\begin{proof}
	From the previous proposition, we know that,
	\begin{equation}
		T_A(\phi_n,\ldots,\phi_n)= \omega_n \phi_n,
		\label{eqn:3:TAinhermite2}
	\end{equation}
	for some $\omega_n$. 
	It it follows that $e^{-it\omega_n}\phi_n(x)$ is a solution of $iu_t = T_A(u,\ldots,u)$.


	Taking the inner product of both sides of \eqref{eqn:3:TAinhermite2} with $\phi_n$ and using \eqref{eqn:3:defnTAimp},
		we find that $\omega_n= 2n H_A(\phi_n)$.
\end{proof}


By applying the symmetries of $E_A$ given in Theorem \ref{thm:3:symmetries} to 
	$\phi_n$, one can obtain other stationary wave solutions.
In fact, with this procedure one finds that all functions of the form,
$
	a e^{ i b x^2  } \phi_n(c x)
$
are stationary waves, where $a\in \C$ and $b,c\in \R$.
If in addition the matrix $A$ satisfies $A(1,\ldots,1)=(1,\ldots,1)$,
	then all functions of the form,
$
	a e^{ i b x^2 + idx } \phi_n(c x+e)
$
are stationary waves, where $a \in \C$ and $b,c,d,e\in \R$.



We note that in higher dimensions, as in the work of \cite{Germain2016},
	the dynamics of the eigenvectors of $H$ under the continuous resonant equation are more interesting because the eigenspaces of $H$ are multidimensional.
	This allows for more complicated dynamics than simply stationary waves.
In dimension one, each eigenspace of $H$ is one dimensional (being spanned by $\phi_n$ alone) and it necessarily follows that
	any eigenvector of $H$ corresponds simply to a stationary wave solution.




\subsection{Classification of the maximizers of the $L^2$ bound}


We have previously established  the inequality $|H_A(f)|\leq \|f\|_{L^2}^{2n}$ and showed that it is sharp.
In this section we discuss the classification those functions that saturate the inequality.
While classifying the cases of equality in an inequality is often illuminating,
	in the theory of Hamiltonians on the phase space $L^2$ it is especially relevant.
In all the Hamiltonian systems discussed in this \thesisor{chapter}{article}, the $L^2$ norm of $f$ is conserved by the Hamiltonian flow, and the Hamiltonian $\Ham$ itself is always conserved. 
Therefore, if one takes as initial data to the flow a function that saturates the inequality $\Ham(f)\leq \|f\|_{L^2}^{2n}$, for all fixed future times $t$
	the solution $x \mapsto f(x,t)$ will still saturate the inequality.
The set of all saturating functions is thus closed under the flow.
Identifying the set of saturating functions can then lead to interesting explicit solutions.
For the Hamiltonians in this \thesisor{chapter}{article}, however, we will find that the saturating functions all correspond simply to stationary wave solutions.

The two examples on \pageref{eqn:3:ex2TA} show that the set of saturating functions for the inequality $|H_A(f)|\leq \|f\|_{L^2}$ 
	will depend on the matrix properties of $A$.
Example \ref{ex:3:1} shows that if $A$ is the identity, or more generally a permutation,
	then the inequality is \emph{always} equality.
If $A$ is a signed permutation, for example the negative of the identity, then
	there is equality if and only if $f$ is even, as we will see.
However if $A$ is not a signed permutation, as in Example \ref{ex:3:2}, 
	then the set of saturating functions is much smaller.

\begin{thm}
	\label{thm:3:maxH}
	Suppose that $A$ is an isometry which is not a signed permutation -- 
		that is, there is some $i$ such that $Ae_i$ is the linear sum of at least two basis elements $e_j$.
	Let $e = (1,\ldots,1)$ denote the vector in $\R^n$ with all its entries 1.
	\begin{enumerate}[label=(\roman*)]
		\item If $Ae=e$, then we have the equality $H_A(f) = \|f\|_{L^2}^{2n}$ if and only if $f(x) = c e^{-\alpha x^2+ \beta x}$ for some $c,\alpha,\beta \in \C$ with $ \Re \alpha>0$.
		\item If $Ae \neq e$, then we have the equality   $H_A(f) = \|f\|_{L^2}^{2n}$  if and only if $f(x) = c e^{-\alpha x^2}$ for some $c,\alpha \in \C$ with $\Re \alpha > 0$.
	\end{enumerate}
\end{thm}
\begin{proof}[Proof of the `if' statements]

	To check the equality case for Gaussians $f(x)=ce^{-\alpha x^2+\beta x}$, we substitute $f$ into both sides of \eqref{eqn:3:cseq},
		which was the equality condition in our use of the \CS{} inequality.
	The left hand side is,
	\begin{align}
		\prod_{k=1}^n f( (Ax)_k ) 
		&=c^n \prod_{k=1}^n \exp\left( - \alpha \langle Ax, e_k \rangle ^2  + \beta\jap{ x,e_k} \right)
		=c^n  \exp \left( - \alpha \sum_{k=1}^n \langle Ax, e_k \rangle^2 + \beta \langle Ax,e_k\rangle \right)		\\
		&=c^n  \exp\left(- \alpha \nrm{Ax}^2 + \beta \langle Ax, e \rangle \right)
		=c^n  \exp\left(- \alpha \nrm{Ax}^2 + \beta \langle x, A^{-1} e \rangle \right),
		\label{eqn:3:cslhs}
	\end{align}
	where in the last line we have used 
		$\langle Ax, e\rangle = \langle x, A^{-1}e \rangle$ coming from $A$ being an isometry.

	An identical computation shows that the right hand side of \eqref{eqn:3:cseq} is,
	$$
		\prod_{k=1}^n f( x_k  ) =
		c^n  \exp \left(  - \alpha \nrm{x}^2 + \beta \langle x, v \rangle \right).
	$$
	If $Ae=e$, so that $e = A^{-1}e$, then both sides are equal for all $c$, $\alpha$ and $\beta$,
		which proves the `if' part of item (i).
	On the other hand, if $Ae \neq e$ then there is an $x\in \R^n$ such that $\langle x, A^{-1}e\rangle \neq \langle x,e \rangle$.
	Hence for equality to hold we necessarily have $\beta=0$.
	However with $\beta=0$ both sides are equal, and so the `if' part of item (ii) is proved.
\end{proof}

The `only if' part of the theorem follows from a more general result that classifies those functions that saturate the multilinear functional inequality
	$|E_A(f_1,\ldots,f_{2n})|\leq \|f_1\|_{L^2}\cdots \|f_{2n}\|_{L^2}$.
	Our classification result, given in Theorem \ref{thm:3:maxE} below, is not new.
	The multilinear functional inequality \eqref{eqn:3:boundonEA} is a specific example of a geometric Brascamp--Lieb inequality.
The Brascamp--Lieb inequalities originated in \cite{Brascamp1976} as generalizations of the H\"{o}lder inequality.
The special class of geometric Brascamp--Lieb inequalities was introduced in \cite{Ball2006},
	and it was subsequently shown, in \cite{Barthe1998}, that they are maximized only for Gaussians.
Theorem \ref{thm:3:maxE} is a special case of this broad result.
Our proof of this special case is, it seems, new, and we think worthy of presentation;
	however, because the result is not new and not essential to other parts of this 
        \thesisor{chapter}{article}, the proof is presented in Appendix A.

%\newpage

\begin{thm}
	\label{thm:3:maxE}
	Let $A$ be an isometry.
	Denote $\tilde{f}_k(x) = f_k(-x)$.
	There exists integers $m$ and $l$, with $0\leq m \leq l \leq n$, and two permutations $\sigma_1$ and $\sigma_2$ of the integers $\{1,\ldots,n\}$
	such that
	\begin{align*}
		E_A&(f_1,\ldots,f_{2n}) =	\\
		&
			\prod_{k=1}^m \jap{f_{\sigma_1(k)}, f_{n+\sigma_2(k)} }
			\prod_{k={m+1}}^l \jap{f_{\sigma_1(k)}, \tilde{f}_{n+\sigma_2(k)} }
			E_B(
				f_{\sigma_1(l+1)},\ldots
				f_{\sigma_1(n)},
				f_{n+\sigma_2(l+1)},\ldots
				f_{n+\sigma_2(n)}),
	\end{align*}
	where the matrix $B:\R^{n-l} \rightarrow \R^{n-l}$ has no permutation part; that is, for all $k$ and $j$, $Be_k \neq \pm e_j$.

	We then have $|E_A(f_1,\ldots,f_{2n})| = \|f_1\|_{L^2}\cdots \|f_{2n}\|_{L^2}$
	if and only if the following three conditions hold.
	\begin{enumerate}
		\item For $k=1,\ldots,m$, $f_{\sigma_1(k)}(x) = C_k f_{n+\sigma_2(k)}(x)$, for some $C_k\in \R$.
		\item For $k=m+1,\ldots,l$, $f_{\sigma_1(k)}(x) = C_k f_{n+\sigma_2(k)}(-x)$, for some $C_k \in \R$.
		\item For $k=l+1,\ldots,n$, $f_{\sigma_1(k)}(x)$ and $f_{n+\sigma_2(k)}(x)$ are Gaussians.
	\end{enumerate}
\end{thm}


\begin{proof}[Proof of the `only if' statements in Theorem \ref{thm:3:maxH}, assuming Theorem \ref{thm:3:maxE}]
	Because $A$ is not a signed permutation, we must have $l<n$ in the notation of Theorem \ref{thm:3:maxE}.
	Then in, Theorem \ref{thm:3:maxE}, condition 3 applies.
	Hence to have the equality $H_A(f)=E_A(f,\ldots,f)=\| f \|_{L^2}^{2n}$, $f$
	must necessarily be a Gaussian.
\end{proof}








\subsection{Regularity of stationary waves: a lemma}

In this final part of our general study of the functional $E_A$, we prove a weight transfer lemma that
	is similar to formula \eqref{eqn:3:weighttrans}.
This lemma will be crucial later to proving that stationary waves of the Hamiltonian systems \eqref{eqn:1:quinticHam} and \eqref{eqn:1:cubicHam} equation are analytic 
	and exponentially decaying once they are in $L^2$.

For fixed $\mu,\epsilon>0$, define,
\[
	%P_{\mu, \epsilon}(x) = \frac{ \mu x^2 }{ 1 + \epsilon x^2}
	%\;\;\text{ and }\;\;
	G_{\mu, \epsilon}(x) = \exp\left( \frac{ \mu x^2 }{ 1 + \epsilon x^2} \right).
\]

\begin{lemma}
	\label{thm:3:weight}
	If $\{ f_k \}_{k=1}^{2n}$ are positive functions, then
	\[
		E_A( f_1,\ldots, f_{2n-1}, f_{2n} \Gmu )
		\leq E_A( f_1\Gmu ,\ldots, f_{2n-1}\Gmu , f_{2n} ).
	\]
\end{lemma}


\begin{proof}
	Define $F_{\mu,\epsilon} = \mu |x|/(1+\epsilon |x|)$.
	We clearly have $ \Gmu(x) = \exp(\Fmu(x^2))$.

	We record two properties of $\Fmu$.
	First, for $x>0$, $\Fmu$ is increasing.
	This may be seen from,
	\[
		\frac{d}{dx}\left( \mu \frac{x}{1+\epsilon x} \right) = \mu \frac{ 1(1+\epsilon x) - x (\epsilon) }{ (1+\epsilon x)^2 }
			=	 \mu \frac{ 1 }{ (1+\epsilon x)^2 } > 0.
	\]
	Next, we have $\Fmu(x_1+x_2) \leq \Fmu(x_1)+\Fmu(x_2)$.
	This may be seen from,
	\begin{align*}
		\Fmu(x_1+x_2) &= \Fmu( |x_1+x_2|) 	
			\leq \Fmu( |x_1| + |x_2|)		
			= \mu \frac{ |x_1| + |x_2| }{ 1 + \epsilon |x_1| + \epsilon |x_2| }	\\
			&\leq \mu \frac{ |x_1| }{ 1 + \epsilon |x_1| }
						+ \mu \frac{ |x_2| }{ 1 + \epsilon |x_2| } = \Fmu(x_1) + \Fmu(x_2).
	\end{align*}

	Now because $A$ is an isometry we have, for all $x\in \R^n$,
	$
		x_n^2 = \sum_{k=1}^n (Ax)_k^2 - \sum_{k=1}^{n-1} (x_k)^2
	$
	and hence by the sublinearity property of $\Fmu$,
	\begin{align*}
		%\Gmu(x_n) &= 
		\Fmu( x_n^2	)	=
		 \Fmu \left( \sum_{k=1}^n (Ax)_k^2 + \sum_{k=1}^{n-1}- (x_k)^2 \right)	
		\leq \sum_{k=1}^n \Fmu( (Ax)_k^2 ) + \sum_{k=1}^{n-1} \Fmu(x_k^2),
	\end{align*}
	Then, because $x \mapsto e^x$ is increasing,
	\[
		\Gmu(x_n) = \exp( \Fmu(x_n^2) ) \leq
			\prod_{k=1}^n \Gmu( (Ax)_k )
			\prod_{k=1}^{n-1} \Gmu( x_k  ).
	\]
	Applying this to $E_A$, we have,
	\begin{align*}
		E_A(f_1,\ldots,f_{2n-1},f_{2n} \Gmu ) &= \int_{\R^n} \left(
		 \prod_{k=1}^{n-1} f_k( (Ax)_k )\of_{n+k} ( x_k ) \right) f_n( (Ax)_n) \of_{2n}(x_n) {\Gmu(x_n) } dx 	\\
			&\leq \int_{\R^n} \left(
		 \prod_{k=1}^{n-1} f_k( (Ax)_k ) \Gmu( (Ax)_k )	\of_{n+k} ( x_k ) \Gmu(x_k)  \right)	\\&\hspace{4cm} f_n( (Ax)_n) {\Gmu((Ax)_n)} \of_{2n}(x_n) dx 	\\
		&=
		E_A(f_1 \Gmu,\ldots,f_{2n-1} \Gmu,f_{2n}  ),
	\end{align*}
	which is what we wanted to prove.
\end{proof}





